Statistical Estimation from Dependent Data

We consider a general statistical estimation problem wherein binary labels across different observations are not independent conditioned on their feature vectors, but dependent, capturing settings where e.g. these observations are collected on a spatial domain, a temporal domain, or a social network, which induce dependencies. We model these dependencies in the language of Markov Random Fields and, importantly, allow these dependencies to be substantial, i.e do not assume that the Markov Random Field capturing these dependencies is in high temperature. As our main contribution we provide algorithms and statistically efficient estimation rates for this model, giving several instantiations of our bounds in logistic regression, sparse logistic regression, and neural network settings with dependent data. Our estimation guarantees follow from novel results for estimating the parameters (i.e. external fields and interaction strengths) of Ising models from a {\em single} sample. {We evaluate our estimation approach on real networked data, showing that it outperforms standard regression approaches that ignore dependencies, across three text classification datasets: Cora, Citeseer and Pubmed.}

==> results.tex <==
\section{Estimation rates - TO BE REMOVED}

We consider two goals. The obvious goal is to recover $\theta^*$ and $\beta^*$, namely, find some $\hat{\theta}$ and $\hat{\beta}$ such that $\|\hat{\theta}-\theta^*\|$ is small. As an intermediate step, we recover $f_{\theta^*}(x_1),\dots,f_{\theta^*}(x_n)$, namely, find $\hat{\theta}$ such that $\sum_{i=1}^n (f_{\theta^*}(x_i)-f_{\hat{\theta}}(x_i))^2$ is small.

\paragraph{Covering numbers}
In order to do so, we need some bound on the covering numbers of $\mathcal{F} = \{f_\theta \colon \theta \in \Theta\}$. For any two $f,f' \in \mathcal{F}$, let $\|f-f'\|_2 = \max_{i=1}^n |f(x_i)-f'(x_i)|$. 
Denote by
$
N(\mathcal{F},\epsilon,2)
$
the minimal cardinality $m$ of a collection of functions $\mathcal{G} \subseteq \mathcal{F}$ such that for all $f\in \mathcal{F}$ there exists $g \in \mathcal{G}$ such that $\|f-g\|_2 \le \epsilon$. 
Define by
\[
N(\mathcal{F},\delta) = C(M) \inf_{\epsilon \ge 0}\lp( 
\log \frac{n}{\delta} +  \epsilon n^{1/2} + \log N(\mathcal{F},\epsilon,2)
\rp).
\]
This is a measure of complexity of the class, that we will use later.
\costis{Give $\epsilon$}
\paragraph{Pointwise complexity}
The rates of estimation will depend on the complexity $N(\mathcal{F})$, however, it will also depend on other complexities of the class, that depend specifically on the matrix $A$ and on $\beta^*$ and $\theta^*$. In particular, define for any $\theta\in \Theta$ and $\beta \in \mathcal{B}$,
\begin{multline*}
\psi(\theta,\beta)
= (\beta^*-\beta)^2 \|A\|_F^2 + \bigg\|f_{\theta^*}(x) - f_{\theta}(x) + \\ (\beta^*-\beta) A \tanh\lp(\frac{\beta^*}{\beta-\beta^*}(f_{\theta^*}(X)- f_{\theta}(X)) + f_{\theta^*}(X)\rp) \bigg\|_2^2.
\end{multline*}

One has the following guarantee:
\begin{theorem}
For any $\delta \ge 0$, w.p. $1-\delta$, the MPLE $(\hat{\theta},\hat{\beta})$ satisfies
\[
\psi(\hat{\theta},\hat{\beta}) \le \mathcal{N}(\mathcal{F},\delta).
\]
\end{theorem}

\paragraph{Deriving estimation rates.}

In order to obtain estimation rates, one can define 
\[
\mathcal{C}_1(r) =
\inf_{\beta \in \mathcal{B},\theta\in \Theta \colon \psi(\beta,\theta)\le r} \frac{1}{n}\|f_{\hat{\theta}}(X)-f_{\theta^*}(X)\|_2^2.
\]
and 
\[
\mathcal{C}_2(r) =
\inf_{\beta \in \mathcal{B},\theta\in \Theta \colon \psi(\beta,\theta)\le r} |\beta-\beta^*|^2.
\]
We have the following:
\begin{theorem}
With probability at least $1-\delta$,
\[
\frac{1}{n}\|f_{\hat{\theta}}(X)-f_{\theta^*}(X)\|_2^2 \le \mathcal{C}_1(\mathcal{N}(\mathcal{F},\delta))
\]
and 
\[
(\hat\beta-\beta^*)^2
\le \mathcal{C}_2(\mathcal{N}(\mathcal{F},\delta)).
\]
\end{theorem}
It is useful to derive bounds on these quantities. One has:
\begin{claim}
It holds that 
\[
\mathcal{C}_1(r), \mathcal{C}_2(r) \le \frac{cr}{\|A\|_F^2}.
\]
\end{claim}
\yuval{Derive the corollaries for regression etc.}

While this bound is very simple, it may be the case that $\|A\|_F$ is small. Even in this situation, it is very likely that $\mathcal{C}_1(r)$ is large. For example, this holds for logistic regression with a random matrix $X$.

\paragraph{A lower bound.}
We show that in fact, 

We have the following statement:
\begin{theorem}
Assume that $\mathcal{B} \subseteq [-(1-\alpha),1-\alpha]$ for some $\alpha \in (0,1)$. Then, there exists $c=c(\alpha,M)$ such that for any estimator $(\hat{\theta},\hat{\beta})$, the minimax rate is at least
\[
\mathcal{C}_1(r).
\]
\end{theorem}

Notice that if the class is convex then $\mathcal{C}_1(a r) \le a \mathcal{C}(r)$ for any $a\ge 0$, hence, this shows some tightness of the bounds: the upper bound is bounded by $\mathcal{C}_1(\mathcal{N}(\mathcal{F},\delta)) \le \mathcal{N}(\mathcal{F},\delta)\mathcal{C}_1(c)/c$,
while the lower bound is
$\mathcal{C}_1(c)$. In particular, if 
Further, we have the following:
\begin{theorem}
Assume that $0 \in \mathcal{B}$. Then, the minimax rate is at least
\[
\mathcal{N}'(\mathcal{F})/n...
\]
(covering numbers ...)
\end{theorem}


-------------------
\begin{theorem} \costis{adde in some way in the intro}
The MPLE $(\hat{\beta},\hat{\theta})$ over $\mathcal{F}$ satisfies w.p. $1-\delta$:
\begin{multline*}
\frac{1}{n} \sum_{i=1}^n (f_{\hat\theta}(x_i)-f_{\theta^*}(x_i))^2 +
|\hat{\beta}-\beta^*|
\\
\le C(M) \frac{\log \frac{n}{\delta} + \inf_{\epsilon \ge 0} \lp(\epsilon n + \log N(\mathcal{F},\epsilon,\infty)\rp)}{\|A\|_F^2} \enspace.
\end{multline*}
\end{theorem}
In order to recover $\theta$, we need the following strong convexity argument. Define
\[
\kappa(\Theta,X)
:= \sqrt{\min_{\theta,\theta' \in \Theta} \frac{\|\theta-\theta'\|^2}{\sum_{i=1}^n (f_\theta(x_i)-f_{\theta'}(x_i))^2/n}}.
\]
Then, trivially 
\[\|\theta-\theta'\| \le \kappa(\Theta,X)\sqrt{\sum_{i=1}^n (f_\theta(x_i)-f_{\theta'}(x_i))^2/n}.\]
It is common to assume that $\kappa(\Theta,X)$ is at least some constant. We derive the following bound for logistic regression:
\begin{corollary} \costis{added in some way in the intro}
Let $R_\theta \ge 0$, let $\Theta = \{\theta \in \mathbb{R}^d \colon \|\theta\|_2 \le R\}$ and let $\max_i \|x_i\|_2 \le R_x$. Then, w.p. $1-\delta$,
\[
\|\hat{\theta}-\theta^*\|_2^2
\le \me^{O(M+R_xR_\theta)}\kappa(\Theta,X)^2 \frac{d \log n + \log(1/\delta)}{\|A\|_F^2}.
\]
\end{corollary} 
For sparse logistic regression, we have the following bound:
\begin{corollary} \costis{added in some way in the intro}
Assume that 
\[\Theta = \{ \theta \in \mathbb{R}^d \colon \|\theta\|_2 \le R_x,\|\theta\|_1 \le s\}
\]
and that $\|x_i\|_\infty \le R_x$. Then, w.p. $1-\delta$,
\begin{multline*}
\|\hat{\theta}-\theta^*\|_2^2
\le \\
\me^{O(M+R_xR_\theta)}\kappa(\Theta,X)^2 \frac{(sn^2\log(d))^{1/3} + \log(1/\delta)}{\|A\|_F^2}.
\end{multline*}
\end{corollary}
We note that both for logistic and sparse logistic regression, the MPLE can be found in polynomial time by convex optimization. 

Finally, we obtain the estimation rates with respect to general classes of functions, for example, neural networks. In this case, it may be impossible to identify $\theta$ given $f_\theta(x_1),\dots,f_\theta(x_n)$. Then, we will care here only for estimating $f_\theta(x_i)$.
\begin{corollary} \costis{added in some way in the intro}
Let $\Theta = [-1,1]^k$, and assume that for any $x$, $f_\theta(x)$ is $L$-Lipschitz in $\theta$, namely, $\|f_\theta(x)-f_{\theta'}(x)\| \le L \|\theta-\theta'\|_\infty$. Then, w.p. $1-\delta$,
\[
\frac{1}{n}\sum_{i=1}^n (f_{\hat{\theta}}(x)-f_{\theta^*}(x))^2
\le \frac{k\log(nL)+\log(1/\delta)}{\|A\|_F^2}\enspace.
\]
\end{corollary}

\yuval{add lower bounds for logistic regression as well, taken from the independent case.}

\yuval{say that $\kappa$ is the minimal eigenvalue of $XX^\top$.}

\yuval{talk about NN}
\subsection{Bounds for small $\|A\|_F$} 

Notice that the above bounds require $\|A\|_F$ to be large. Indeed, in some cases this is necessary. However, in many cases it isn't and that's the goal of this section. We derive a more general theorem:
\begin{theorem}
Denote for $\lambda \in \mathbb{R}$ and $\theta \in \Theta$,
\begin{multline*}
Q(\theta,\lambda) = \|\lambda A\|_F^2 +\\ \lp\|\frac{h^* - h}{\|h^* - h\|} - \lambda A \tanh\lp(\frac{\beta^*}{\lambda}\frac{h^* - h}{\|h^* - h\|} + h^*\rp)\rp\|_2^2.
\end{multline*}
With probability $1-\delta$,
\begin{multline*}
    \frac{1}{n}\sum_{i=1}^n (f_{\hat{\theta}}(x_i)-f_{\theta^*}(x_i))^2\le \\
    C(M)
    \frac{\log \frac{n}{\delta} + \inf_{\epsilon \ge 0} \lp(\epsilon n + \log N(\mathcal{F},\epsilon,\infty)\rp)}{n\inf_{\lambda \in \R, \theta \in \Theta}Q(\theta,\lambda)}\enspace.
\end{multline*}
\end{theorem}

Similarly, we have a rate for $\beta$. While the quantity $Q(\theta,\lambda)$ is always bounded by the Forbenuis norm, we show that it also can be bounded for a random regression instance:
\begin{corollary}
Add the theorem.
\end{corollary}

\subsection{Lower bound}

In fact, the upper bound is tight.
